Accelerating Psychometric Screening Tests With Bayesian Active Differential Selection

Classical methods for psychometric function estimation either require excessive measurements or produce only a low-resolution approximation of the target psychometric function. In this paper, we propose a novel solution for rapid screening for a change in the psychometric function estimation of a given patient. We use Bayesian active model selection to perform an automated pure-tone audiogram test with the goal of quickly finding if the current audiogram will be different from a previous audiogram. We validate our approach using audiometric data from the National Institute for Occupational Safety and Health NIOSH. Initial results show that with a few tones we can detect if the patient's audiometric function has changed between the two test sessions with high confidence.

==> content/related_work.tex <==
% !TEX root = ../neurips_2019.tex

\section{Related work} 

Prior work using \acro{GP}s for audiogram estimation have proposed a variant of uncertainty sampling that selected points with maximum variance \cite{Song:2015}. This work increased both the speed and accuracy of the standard threshold audiogram estimation by at least an order of magnitude. In \cite{Gardner:2015}, a framework called Bayesian Active Model Selection (\acro{BAMS}) was proposed to quickly distinguish which of a number of predetermined models best explains a function being actively observed. \acro{BAMS} was applied to rapid screening for noise-induced hearing loss.

Both of the aforementioned papers explored the use of machine learning audiometry in one ear, this approach was extended to exploit the shared variance between ears using a conjoint audiogram \cite{Barbour2019, DiLorenzo2017ConjointAE}. Learning the audiogram for both ears was shown to be as fast as, or sometimes faster than, learning a single ear individually. 

Our work is complementary to the methodologies described above. Instead of ignoring prior information from the individual or a similar individual, we proposed starting our current test acknowledging a previous audiometric test might be available to reference. The underlying psychometric function that the audiogram is meant to estimate is correlated with previous audiometric tests that the subject has taken, as well as other audiometric tests more generally. In the same way that conjoint audiogram estimation utilizes covariance between ears to reduce the number of tones needed to estimate the underlying function, we propose a novel approach for determining whether two audiograms represent the same or a different psychometric function.
